TipTop: (Almost) Exact Solutions for Influence Maximization in Billion-scale Networks

In this paper, we study the Cost-aware Target Viral Marketing (CTVM) problem, a generalization of Influence Maximization (IM). CTVM asks for the most cost-effective users to influence the most relevant users. In contrast to the vast literature, we attempt to offer exact solutions. As the problem is NP-hard, thus, exact solutions are intractable, we propose TipTop, a $(1-\epsilon)$-optimal solution for arbitrary $\epsilon>0$ that scales to very large networks such as Twitter. At the heart of TipTop lies an innovative technique that reduces the number of samples as much as possible. This allows us to exactly solve CTVM on a much smaller space of generated samples using Integer Programming. Furthermore, TipTop lends a tool for researchers to benchmark their solutions against the optimal one in large-scale networks, which is currently not available.

==> body/sampling.tex <==
\section{Benefit-aware Reverse Influence Sampling}
	
	In this section, we show that the well-studied convectional sampling strategy, called Reverse Influence Sampling (RIS), does not work well in \CTVM{} problem when we have benefit. In fact, straightforwardly applying RIS to \CTVM{} may lead to an extremely inefficient algorithm with the number of samplings being up to $n$ times the number needed for \IM{} task. Therefore, we propose an adapted version of RIS, named Benefit-aware Reverse Influence Sampling (\BRIS{}), for estimating expected benefit.
	
	\subsection{Summary of the RIS  method}
	
	Borgs et al. \cite{Borgs14} introduced a novel approach, called Reverse Influence Sampling (RIS), to estimate the influence in IC model. RIC generates a hypergraph $\mathcal H$ consisting of random hyperedges where each hyperedge $\mathcal E_j$ is constructed as follows. First, a node $u$ is chosen uniformly at random and then they travel in the \emph{reversed graph} to infer which nodes can influence $u$. Repeating that process multiple times will provide us with information on the influence landscape of the network. In $\mathcal H$, the degree of a set $S \in V$ is defined as $deg_{\mathcal H}(S) = |\{\mathcal E | \mathcal E \cap S \neq \emptyset\}|$. Intuitively, if node $u$ has higher influence to other people than node $v$, with high probability, node $u$ will appear more often in a random set of hyperedges than node $v$. The other direction is also very inherent. The following lemma (see \cite{Borgs14} for details) capture this intuition
	
	\begin{lemma}
		For each subset of nodes $S\in V$,
		\begin{align}
			\I(S) = n \Pr[\mathcal E \cap S \neq \emptyset]
		\end{align} where $\mathcal E$ is a random hyperedge.
       
	\end{lemma}
	Thus, the problem of estimating the influence of a subset $S$ ($\I(S)$) is transformed into the problem of estimating $\Pr[\mathcal E \cap~S \neq \emptyset]$. Based on this result, the framework of using RIS for \IM{} problem consists of two steps:
	\begin{itemize}
		\item Generate a sufficiently large random hyperedges using RIS to capture the influence landscape in the network.
		\item Find a seed set that covers the maximum number of hyperedges by using greedy approach on hyperedges.
	\end{itemize}
	In the first step, with the number of hyperedges
	\begin{align}
		\label{eq:tim_edge}
		\theta = (8 + 2\epsilon)\frac{n (\ln n + \ln {n \choose k} + \ln 2)}{OPT_k \epsilon^2},
	\end{align}
	TIM/TIM+ \cite{Tang14} return a $(1 - 1/e -\epsilon)$-approximate solution with probability $1/n$.
	
    
	We, now, determine the number of samples required to approximate accurately a fixed subset $S \in V$ with high probability. If we define i.i.d. random variables $X_1,...,X_T$ having mean value ~$\E[{X_i}]= \mu = \Pr[\mathcal E \cap S \neq \emptyset] = \frac{\I(S)}{n}$, then an estimation of $\I(S)$ is given by
	\begin{align}
		\hat \I(S) = n \hat \Pr[\mathcal E \cap S \neq \emptyset] = \frac{\sum_{i=1}^{T}X_i}{T}n = \frac{deg_{\mathcal H}(S)}{T}n.
	\end{align}
	where hypergraph $\mathcal H$ contains $T$ hyperedges. However, how large $T$ have to be in order to approximate $\Pr[\mathcal E \cap S \neq \emptyset]$ accurately. The following lemmas provide us the number of samples needed to bound approximation error.
%	The LT and IC models are equivalent to the reachability in their corresponding \emph{live-edge} graphs, defined in \cite{Kempe03}: In LT model, given a graph $\mathcal G = (V, E, w)$, for every $v \in V$, select at most one of its incoming edges at random, such that the edge $(u, v)$ is selected with probability $w(u, v)$, and no edge is selected with probability $1 - \sum_{u} w(u, v)$. In contrast, each edge $(u, v)$, under IC model, is selected independently with probability $w(u,v)$. Each live-graph $G$ generated from $\mathcal G$ is also called a sample graph. The influence spread of a seed set $S$ is same as the expected number of nodes reachable from $S$ over all possible sample graphs.
	
%	They provide an approximation algorithm which requires at least $48  \frac{m+ n \log n}{\epsilon^3 \I(S_{opt})} $ sampling times and has approximation factor of $1 -1/e-\epsilon$ for \IM{} problem. Most recently, Tang et al.'s \cite{Tang14} needs only $(8+\epsilon) \frac{k(m+n)}{\epsilon^2 \I(S_{opt})}$ hyperedges to provide the same guarantees.  Here $S_{opt} =  \max_{|S| = k, S \subseteq V} \{ \I(S) \}$, the maximum influence of any size-$k$ seed set. Hence, the Tang et al.'s  is asymptotically $\frac{1}{\epsilon}\log n$ times faster than the Borgs et al's.
%	However, RIS works well for \IM{} problem but \CTVM{} due to the added constraints of node benefit as shown subsequently. We will, first, summarize the framework of TIM+, the fastest \IM{} method with provable approximation guarantee, using RIS and then demonstrate that the intuitive adaption of TIM+ to \CTVM{} always requires more samples than that for \IM{} problem and, in the worst case, it needs $n$ times more samples. 
	
%	Basically, the methods in \cite{Borgs14,Tang14} include two main steps: 
%	\begin{itemize}
%		\item Generate a certain number of hyperedges by RIS sampling to guarantee that
%		\begin{align}
%		\label{eq:tim+_gua}
%		\Pr[|\hat \I(S_k) - \I(S_k)| \ge \epsilon \I(S_{opt})] \le 1 - \delta 
%		\end{align} for any size-$k$ set where $\hat \I(S_k) = \frac{deg_{\mathcal{H}}(S_k)}{m_{\mathcal{H}}}n$ and $\I(S_{opt}) =  \max_{|S| = k} \{ \I(S) \}$, the maximum influence of any size-$k$ seed set. 

%Borgs et al.'s method requires at least $48  \frac{m+ n \log n}{\epsilon^3 \I(S_{opt})} $ sampling times while  Tang et al.'s \cite{Tang14} needs only $(8+\epsilon) \frac{k(m+n)}{\epsilon^2 \I(S_{opt})}$ hyperedges;
		
%		\item Apply greedy algorithm for Max-coverage problem to select top $k$ nodes to cover the maximum number of hyperedges. 
%		
%	\end{itemize}
%	As shown in \cite{Tang14}, the sampling step is the most expensive and decides the complexity of the algorithm. Analogously, the number of samples contributes most to the complexity and the method requiring fewer samples takes advantages. 
	
	\begin{lemma}
		\label{lem:error_bound}
		Let $X_1,..., X_T$ be i.i.d. random variables with $\E[{X_i}] = \mu $. For any fixed $T > 0$,
		\[
		\Pr[\hat \mu \geq  (1+ \epsilon) \mu] \leq
		e^{\frac{-T\mu\epsilon^2}{2c }}
		\]
		and
		\[
		\Pr[\hat \mu \leq  (1- \epsilon) \mu] \leq e^{\frac{-T\mu\epsilon^2}{2c }}.
		\]
		where $\hat \mu = \frac{\sum_{i = 1}^T X_i}{T}$.
	\end{lemma}
	
	\begin{lemma}
		\label{lem:sub_opt_sample}
		Given $0 \le \epsilon \le 1$ and $0 \le \delta \le 1$, if we have
		\begin{align}
		\label{eq:sub_opt_sample}
		T = 2c \ln( \frac{2}{\delta})  \frac{1}{\epsilon^2 \mu}
		\end{align}
		i.i.d. random variables $X_1,...,X_T$ with $\mu_{X_i} = \mu$ then
		\begin{align}
		\label{eq:eps_del_app}
		\Pr[|\hat \mu - \mu| \ge \epsilon \mu] \geq 1 - \delta
		\end{align}
	\end{lemma}
	
	The probability in \ref{eq:eps_del_app} is called $(\epsilon, \delta)$-approximation. Lemma \ref{lem:error_bound} is a tight version of Chernoff-Hoeffding theorem and Lemma \ref{lem:sub_opt_sample} is the Generalized Zero-One Estimator Theorem (See \cite{Dagum00} for both). Applying Lemma \ref{lem:error_bound} to the approximation of $\Pr[\mathcal E \cap~ S \neq~ \emptyset]$, we find that
	\begin{align}
		\label{eq:num_sam_tim+}
		T = 2c\ln(23/\delta) \frac{1}{\epsilon^2\mu_{X_i}} = 2c\ln( \frac{2}{\delta}) \frac{n}{\epsilon^2\I(S)}.
	\end{align} is the sufficient number of samples to guarantee
	\begin{align}
		\Pr[| \hat \I(S) - \I(S)| \le \epsilon \I(S)] \geq 1 - \delta
	\end{align}
	
	Thus, the most straightforward way of using RIS on \CTVM{} problem, where node $u$ has a benefit $b(u)$, is to define i.i.d. random variables $X'_1, ..., X'_n$ with mean $E[{X'_i}] = \frac{\B(S)}{n}=\frac{\sum_{v\in V}\I(S,v)b(v)}{n}$ and a sample corresponds to $1_{(S\cap \mathcal{E}_v \neq \emptyset)}b(v)$ where $v$ is random. However, this intuitively adapted algorithms requires the number of samples up to $n$ times larger than that for \IM{} problem as shown by the following lemma with the proof in the Appendix.
	
	\begin{lemma}
		\label{lem:sample_ris}
		The naive algorithm using RIS sampling for \CTVM{} problem requires
		\begin{align}
		\label{eq:num_sam_tim+_ada}
		T' = 2c\ln( 2/\delta) \frac{nb_{max}}{\epsilon^2\B(S)}
		\end{align} samples to estimate expected benefit of a set $S$.
	\end{lemma}
	
	Comparing $T$ in \ref{eq:num_sam_tim+} and $T'$ in \ref{eq:num_sam_tim+_ada}: 1) In case of Influence Maximization problem where all nodes have the same benefit of 1, $T = T'$; 2) In the worst case where $b_{max} = n$ and $\B(S) = O(\I(S))$, then the adapted TIM+ to \CTVM{} requires $n$ times that number for \IM{} problem.
	
	\subsection{Efficient Sampling Strategy for \CTVM{}}
	
	Due to the inefficiency of RIS in \CTVM{}, we propose an efficient adapted version of RIS, called Benefit-aware Reverse Influence Sampling (\BRIS{}), for estimating expected benefit of a seed set. The \BRIS{} procedure to generate a random hyperedge $\mathcal E_j \subseteq V$ under LT model is summarized in Algorithm \ref{alg:RIS}. A procedure for IC model can be similarly constructed. The great deal of difference of \BRIS{} is where we choose the starting node proportional to node benefit as opposed to choosing uniformly at random in RIS. That is the probability of choosing node $u$ is $P(u) = \frac{b(u)}{\sum_{v \in V} b(v)} = \frac{b(u)}{\Gamma}$. After choosing a starting node $u$, we attempt to select an \emph{in-neighbor} $v$ of $u$, i.e. $(v, u)$ is an edge of $\mathcal G$, according to the edge weights. Then we ``move'' to $v$ and repeat, i.e. to continue the process with $v$ replaced by $u$. The procedure stops when we encounter a previously visited vertex or no edge is selected. The hyperedge is then returned as the set of nodes visited along the process.
	
	\begin{algorithm}
		\caption{Benefit-aware Reverse Influence Sampling under LT model (\BRIS-LT) }
		\label{alg:RIS}
		\begin{algorithmic}
			\State {\textbf{Input}: Weighted graph $\mathcal G=(V, E, w)$}
			\State {\textbf{Output}: A random hyperedge $\mathcal E_j \subseteq V$.}
			
			\State 1: $\mathcal E_j \leftarrow  \emptyset$
			\State 2: Pick a node $u$ with probability $\frac{b(u)}{\Gamma}$. 
			\State 3: \textbf{Repeat}
			\State 4: \text{  \   }	 Add $u$ to $\mathcal E_j$
			\State 5:	\text{  \   } Attempt to select an edge $(v, u)$ using live-edge model
			\State 6: \text{  \   } \textbf{if} edge $(v, u)$ is selected \textbf{then} Set $u \leftarrow v$.
			\State 7: \textbf{Until} ($u \in \mathcal E_j$) OR (no edge is selected)
			\State 8: Return $\mathcal E_j$
		\end{algorithmic}
	\end{algorithm}
	
	The key insight into why random hyperedges generated via \BRIS{} can capture the benefit landscape is stated in the following lemma. 
	\begin{lemma}
		\label{lem:ris}
		Given a fixed seed set $S \subseteq V$, for a random hyperedge $\mathcal E$,
		\[
		\Pr[ \mathcal 	E \cap S \neq \emptyset ] = \frac{\B(S)}{\Gamma}
		\]
	\end{lemma}
	\textit{Proof}.
		\begin{align}
			\label{eq:needed_samples}
			\B(S) &= \sum_{u\in V} \Pr[ \text{ u is reachable from a node in }S ]b(u) \nonumber \\
			&= \sum_{u \in V} \Pr[\exists v\in S \text{ such that } v \in \mathcal E(u) ]b(u)\nonumber \\
			&= \Gamma\sum_{u \in V} \Pr[\exists v\in S \text{ such that } v \in \mathcal E(u) ]\frac{b(u)}{\Gamma} \nonumber \\
			&= \Gamma\Pr[\exists v\in S \text{ such that } v \in \mathcal E ] \nonumber \\
			&= \Gamma \Pr[S\cap \mathcal E \neq \emptyset]
		\end{align}
	The transition from the third to forth equality follows from the distribution of choosing node $u$ as a starting node of \BRIS{}. We select $u$ with probability $P(u) = \frac{b(u)}{\Gamma}$, hence, the forth equality contains the expected probability taken over the node benefit distribution.
	
	Now, we analyze the number of samples needed to $(\epsilon, \delta)$-approximate a random set $S$. First, define variable $X = 1_{(S\cap \mathcal E \neq \emptyset)}$ where $\mathcal E$ is a random hyperedge with the mean value $\mu = \Pr [S\cap \mathcal E] = \frac{\B(S)}{\Gamma}$ (followed by Eq. \ref{eq:needed_samples}). Thus, applying Lemma \ref{lem:sub_opt_sample} gives
	\begin{align}
		\label{eq:bct_sample}
		T = 2c\frac{\Gamma \ln 2/\delta}{\epsilon^2\B(S)}.
	\end{align}
	This number of samples is asymptotically optimal based on the results in \cite{Dagum00}. By comparing Eq. \ref{eq:bct_sample} with Eq. \ref{eq:num_sam_tim+_ada}, we see that algorithm using \BRIS{} requires up to $n$ times fewer samples than the straightforward strategy.
